The Role of PDE-Based Parameterization Techniques in Gradient-Based IGA Shape Optimization Applications

This paper proposes a shape optimization algorithm based on the principles of Isogeometric Analysis (IGA) in which the parameterization of the geometry enters the problem formulation as an additional PDE-constraint. Inspired by the isoparametric principle of IGA, the parameterization and the governing state equation are treated using the same numerical technique. This leads to a scheme that is comparatively easy to differentiate, allowing for a fully symbolic derivation of the gradient and subsequent gradient-based optimization. To improve the efficiency and robustness of the scheme, the basis is re-selected during each optimization iteration and adjusted to the current needs. The scheme is validated in two test cases.

==> sec_intro_secure_copy.tex <==
% !TEX root = ./main.tex
%!TeX spellcheck = en-US
\section{Introduction}
\label{sect:Introduction}
\textit{This introduction is taken from another paper and has to be adjusted to the topic of this manuscript.}\\[0.5cm]
Isogeometric analysis (IgA), first introduced by Hughes et al. in \emph{[citation forthcoming]}, is a numerical technique that aims to bridge the gap between computer aided design (CAD) and (isoparametric) finite element analysis (FEA). This is accomplished by building the geometry mapping from the same spline basis that is used to approximately solve PDE-problems posed over the geometry. As such, spline-based parameterization techniques have received an increased amount of interest in the mathematical community in recent years. Since the CAD pipeline typically provides no more than a spline-based description of the boundary contours of the target geometry, the purpose of all parameterization algorithms is to generate a bijective (folding-free) geometry parameterization from the boundary CAD data. Analogous to mesh quality in classical FEA, the parameteric quality of the surface parameterization has a profound impact on the numerical accuracy of the isogeometric analysis \emph{[citation forthcoming]}. Therefore, besides bijectivity, proficient parameterization algorithms aim at generating parameterizations of high numerical quality. \\
One of the most important applications of IgA lies in shape-optimization problems. Since the geometry changes at every shape optimization iteration, algorithms that are differentiable with respect to the design variables (i.e., the boundary control points) have a further advantage since they allow for employing gradient-based shape-optimization algorithms which tend to converge in fewer iterations than their zeroth-order counterparts. Another advantage of differentiability is efficiency: as the inner control points are a smooth function of the boundary control points, there is no need for full remeshing after each iteration since cheaper mesh update strategies can be employed. This is also true for settings in which the boundary contours change as a smooth function of time. \\
Traditionally, parameterizations for IgA-applications are built from tensor-product spline spaces. Unfortunately, structured spline technologies do not allow for local refinement as knot-insertion in one parametric direction automatically refines a whole row / column of the underlying spline space. For the geometry description, this may result in a very dense spline basis whenever many degrees of freedom (DOFs) are required to properly resolve the boundary contours. As a result, the total number of unknowns (the inner control points) may become infeasibly large, leading to a severe slow-down of the meshing process and / or the isogeometric analysis. \\
To address above efficiency concerns, this paper introduces a PDE-based planar parameterization framework that uses THB-splines \emph{[citation forthcoming]}, an unstructured spline-technology which allows for local refinement, potentially reducing the required total number of DOFs. A major challenge of unstructured spline technologies is deciding where local refinement is required and where a lower resolution suffices. For this, we employ the principles of \textit{dual weighted residual} (DWR) \emph{[citation forthcoming]}, an a posteriori refinement technique for PDE-problems based on duality considerations. Furthermore, we augment the problem formulation with a mechanism that allows for changing the parametric properties of the PDE-solution in order to fine-tune the parametric properties of the mapping operator.
